Advances in Data-Driven Analysis and Synthesis of 3D Indoor Scenes

This report surveys advances in deep learning-based modeling techniques that address four different 3D indoor scene analysis tasks, as well as synthesis of 3D indoor scenes. We describe different kinds of representations for indoor scenes, various indoor scene datasets available for research in the aforementioned areas, and discuss notable works employing machine learning models for such scene modeling tasks based on these representations. Specifically, we focus on the analysis and synthesis of 3D indoor scenes. With respect to analysis, we focus on four basic scene understanding tasks -- 3D object detection, 3D scene segmentation, 3D scene reconstruction and 3D scene similarity. And for synthesis, we mainly discuss neural scene synthesis works, though also highlighting model-driven methods that allow for human-centric, progressive scene synthesis. We identify the challenges involved in modeling scenes for these tasks and the kind of machinery that needs to be developed to adapt to the data representation, and the task setting in general. For each of these tasks, we provide a comprehensive summary of the state-of-the-art works across different axes such as the choice of data representation, backbone, evaluation metric, input, output, etc., providing an organized review of the literature. Towards the end, we discuss some interesting research directions that have the potential to make a direct impact on the way users interact and engage with these virtual scene models, making them an integral part of the metaverse.

==> 4-3D_scene_analysis.tex <==
\section{3D scene analysis}
\label{sec:analysis}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\linewidth, height=0.7\linewidth]{Figures/scene_analysis/object_detection/sliding_shapes.pdf}
    \caption{Illustration of training (top) and test (bottom) phases for 3D object detection using \emph{Sliding Shapes} \cite{song2014sliding}. Refer to the text in Section \ref{subsec:obj_det} for details.}
    \label{fig:sliding_shapes}
    \vspace{-15pt}
\end{figure}

% Indoor environments (ex: office spaces, living rooms) form an essential part of our lives and are characterized by the type of furniture that go in such spaces, which are, in turn, determined by human actions. 
% %
% The ubiquity of indoor scenes has necessitated the development of virtual models for simulating real-life experience in video games, robot navigation and virtual/augmented reality (VR/AR) applications.
% %
% The composition of such environments varies considerably based on the human activities they are designed to serve. 
% %


% Manually designing such scenes is time-consuming and expensive as it requires expertise in interior design and familiarity with the design tools. Computational algorithms that can achieve results with comparable fidelity are necessary to overcome this content-creation bottleneck. %, and also for wider adoption of such technology in different domains. 
% To this end, many 3D indoor scene synthesis works have been proposed in the last decade that use example-based, probabilistic approach \cite{merrell2011interactive, yu2011make, fisher2012example, xu2013sketch2scene, fisher2015activity, ma2016action, ma2018language} for synthesizing scenes. With the rapid advancement in machine learning techniques, recent works \cite{wang2018deep, li2019grains, zhou2019scenegraphnet, zhang2020deep, nie2020total3dunderstanding} have taken a data-driven learning-based approach toward scene synthesis.\\
% %
% \newline
%
\input{Tables/3d_obj_det}
The first step in computational scene synthesis, i.e., teaching computers to generate indoor environments, is scene analysis, i.e., teaching computers to understand their composition -- what characterizes scenes of a particular category (say, bedrooms), what kind of furniture goes in there, how to identify different furniture objects, how to detect different instances of the same object in the scene, and how to reason about their placements in the context of global scene plausibility. In other words, computational analysis of scenes, a.k.a scene understanding, is a prelude to scene synthesis. 

Understanding comes from observations, which are relayed by indoor scene datasets, which have been discussed in Section \ref{sec:dataset_list}. %such as SUN \cite{xiao2010sun}, NYU RGB-D \cite{silberman11indoor, Silberman:ECCV12}, SUN RGB-D \cite{song2015sun}, ScanNet \cite{dai2017scannet}, SUNCG \cite{song2017semantic}, Matterport3D \cite{chang2017matterport3d}, Structure3D \cite{zheng2020structured3d}, 2D-3D Semantic Scene dataset (S3DIS) \cite{armeni2017joint}, HyperSim \cite{roberts2020hypersim} and 3D-FRONT \cite{fu20213d} to name a few. 
Each of these datasets uses a different form of representation for indoor scenes, as categorized in Section \ref{sec:layout_reps}. In literature, different scene analysis tasks use different kinds of representation, which could be motivated by different factors such as the easy availability of a dataset with one form of representation, friendliness toward off-the-shelf networks used as a part of the proposed approach, or the need for developing novel architectures due to the choice of a certain representation. In the upcoming sections, we provide a summary of different works along similar axes. \\
%

%
The main analysis tasks we cover in this report include 3D object detection (Section \ref{subsec:obj_det}), semantic scene segmentation (Section \ref{subsec:3d_ssg}), 3D scene reconstruction (Section \ref{subsec:scene_recon}, and 3D scene similarity (Section \ref{subsec:scene_sim}).

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\linewidth, height=0.7\linewidth]{Figures/scene_analysis/object_detection/deep_sliding_shapes.pdf}
    \caption{Figure illustrating the technique behind \emph{Deep Sliding Shapes} \cite{song2016deep}. Top: using a 3D CNN to propose regions of interest in 3D. Bottom: training pipeline based on the 3D and 2D CNNs to localize bounding boxes in 3D space. }
    \label{fig:deep_sliding_shapes}
    \vspace{-15pt}
\end{figure}

\subsection{3D object detection}
\label{subsec:obj_det}
%
Recognizing objects in a scene, i.e., identifying their semantic category and localizing their spatial position via 2D/3D bounding boxes has been a fundamental and long-standing goal of computer vision. This report does \emph{not} cover works on 2D object detection in RGB images. Rather, we focus on notable works on 3D object detection in indoor scenes, a task that is challenging mainly due to variations in shape (both inter and intra-class), texture, illumination, viewpoint, and the presence of clutter and occlusions. Table \ref{tab:3d_object_detection_works} provides a comprehensive overview of notable methods on 3D object detection in indoor scenes. Broadly, these works can be categorized into three types: sliding window techniques \cite{song2014sliding, song2016deep}, grouping techniques \cite{qi2019deep,qi2020imvotenet, xie2020mlcvnet}, and group-free techniques \cite{liu2021group}, as discussed below.

\textbf{Sliding window techniques.}
Song et al. \cite{song2014sliding} introduce Sliding Shapes, a supervised machine learning-based approach for 3D object detection. The work makes use of depth maps for designing a 3D object detector, in addition to a collection of 3D CAD models, where each CAD model is rendered from many viewpoints, obtaining synthetic depth maps for every viewpoint. For each depth rendering of a CAD model, features based on truncated sign distance fields (TSDF) values, 3D normals, point density, and voxel occupancy are extracted (collectively known as point features) and an exemplar support vector machine (Exemplar-SVM) classifier is trained on point features of the sensor-acquired scenes. During test time, a sliding window is moved through the 3D scene space to detect an object; see Fig \ref{fig:sliding_shapes}. 

The successor to Sliding Shapes, termed, Deep Sliding Shapes, was presented in \cite{song2016deep}. It is a supervised deep learning-based framework which makes use of a 3D ConvNet that takes a 3D volumetric scene from an RGB-D image as input and outputs 3D object bounding boxes. A 3D Region Proposal Network (RPN) is trained at two different scales to learn object-ness from geometric shapes. An Object Recognition Network (ORN) is \emph{jointly} trained with RPN to extract geometric features in 3D and color features in 2D, to eventually output a category label and 3D box coordinates. Figure \ref{fig:deep_sliding_shapes} illustrates these two steps during training. At test time, a sliding window is again moved through the space of a 3D scene to detect the presence of an object.

One main limitation of both the above approaches is that they do not explicitly encode object orientation, which can hurt the performance of a 3D object detection system. Ren et al. \cite{ren2016three} overcome this limitation by designing a new set of features, called, cloud-of-oriented-gradient (COG), that robustly link 3D object pose to 2D image boundaries. COG features are nothing but the gradients of 2D projections of oriented cuboid points falling inside the object voxel. COG features, in addition to the point cloud density features and 3D normal histogram features form the point features, are used to train an SVM for 3D object detection similar in spirit to Sliding Shapes. Sedaghat et al. \cite{sedaghat2016orientation} also address the limitation of Deep Sliding Shapes by adding orientation classification as an auxiliary task, and demonstrate that speed and accuracy of 3D detection using a sliding window increases when the 3D CNN is jointly trained on object labels, location and pose.

\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth, height = 0.6\linewidth]{Figures/scene_analysis/object_detection/VoteNet.pdf}
    \caption{An end-to-end learning pipeline for 3D object detection using voting technique (\emph{VoteNet}) \cite{qi2019deep} that directly operates on 3D data without the need for any 2D image priors, such as 2D object detectors. }
    \label{fig:vote_net}
    \vspace{-15pt}
\end{figure}

\textbf{Voting techniques.}
In recent years, voting concepts, specifically, Hough voting, have made a comeback in the space of 3D object detection. VoteNet \cite{qi2019deep} and ImVoteNet \cite{qi2020imvotenet} are two such works that are built on voting strategies. 
VoteNet demonstrates two advantages of using the voting strategy for 3D object detection -- first, it does not make use of any 2D object detectors which used to be the de-facto step in 3D object detection, and second, the Hough voting technique used in the work is now differentiably learned in an end-to-end supervised manner. 
%

%
As shown in Figure \ref{fig:vote_net}, the input to the system is a colorless point cloud of a scene, which is processed by PointNet++ \cite{qi2017pointnet++}, to produce features for every point. A voting net, which is nothing but a MLP on these point features, produces virtual points, called votes, for centers of 3D bounding boxes. The votes are clustered in the 3D space using farthest point sampling and L$_2$ distance, from where the extent of the 3D bounding boxes and their centroids are regressed using another MLP. All of this training is done in a supervised manner, where the votes on the training data are available since it is supervised. ImVoteNet \cite{qi2020imvotenet} incorporates all the steps from VoteNet, but in addition, makes use of a 2D object detector, where votes are obtained in the image space, which is lifted to the 3D space (along with the 2D object center) by ray-casting.%, and the difference in displacements is learned in a supervised manner.\\

\textbf{Hybrid technique.}
A hybrid model for 3D object detection on colorless scene point clouds was proposed by Zhang et al. \cite{zhang2020h3dnet}, where bounding boxes are represented using three geometric primitives -- bounding box centers, face centers, and edge centers. These hybrid geometric primitives represent an overcomplete set of constraints that are predicted using a neural network. The predicted geometric primitives are converted into object proposals by defining a distance function between an object and the geometric primitives. The main purpose served by the distance function is that it helps in the continuous optimization of object proposals. A final matching and refinement module is proposed to classify object proposals into detected objects.

\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth, height = 0.6\linewidth]{Figures/scene_analysis/segmentation/pointnet_pic.PNG}
    \caption{\emph{PointNet} architecture \cite{qi2017pointnet} that was originally proposed for the task of shape classification and segmentation at the object part level, as well as for indoor scenes. This work has been the basis for many 3D object detection works, especially for developing task-specific feature descriptors.}
    \label{fig:point_net}
    \vspace{-15pt}
\end{figure}

% \agp{
\revision{
\textbf{Context-aware techniques.}
Despite a large inter- and intra-class shape variation and illumination effects in 3D indoor scenes, the context relation of object arrangements provides useful cues for object detection. Some prior works seek holistic scene understanding to improve object detection with other auxiliary tasks. For example, Lin et al.~\cite{LinFU13} first estimate the candidate 3D cuboids of the objects, and then use a conditional random field (CRF) model to \emph{jointly} solve for the scene classification and 3D object recognition. This holistic approach takes the scene context into account while also accounting for relations between different objects for the task of object classification. 

Zhang et al.~\cite{ZhangBKIX17} integrates the context relations into neural networks using automatically constructed scene templates. They first select a template and align it with the input scene by a transformation network, and then compute the global and local features of the input scene based on the aligned template. What makes this approach holistic is that it uses global features to classify scenes, while using both the global and local features to predict the existence of objects and the box offset for better alignment. Huang et al.~\cite{huang2018cooperative} refer to their approach of jointly recovering the object bounding boxes, room layout, and camera pose as a holistic one. They estimate all this information from a given RGB image, then use the predicted camera pose to project the inferred 3D bounding boxes back to the 2D plane, in order to obtain a more consistent prediction.

Recent investigations have looked into utilizing context information to complement 3D object detection. Feng et al.~\cite{FengGWZM21} take PointNet++~\cite{qi2017pointnet} as the backbone to generate candidate 3D object bounding boxes, and then use the object-object relation graph to reduce uncertainty during 3D bounding box regression. Duan et al.~\cite{Duan0LYL022} argue that 3D object detection can be improved by adopting relations between representative proposals, which is more efficient than those between all the predicted proposals. They accomplish this by proposing what they call a DisARM module, which first samples relation anchors with rich information and then estimates the weight of each proposal w.r.t the anchors based on spatial- and feature-aware displacements. The weighted proposal-anchor features provide contextual information to complement the anchor proposal feature. In addition, Sun et al.~\cite{0003FZLL22} propose an online data augmentation pipeline based on the functional relation between objects, called Correlation Field, that helps boost the performance of object detection.
% }
}

\textbf{Transformer-based techniques.}
A more recent supervised learning approach by Liu et al. \cite{liu2021group} to 3D object detection on scene point clouds makes use of the transformer model \cite{vaswani2017attention}, which is essentially an attention-based feature aggregation module on the input. Unlike voting-based object detection works such as VoteNet \cite{qi2019deep} and ImVoteNet \cite{qi2020imvotenet} where the points are assigned to an object candidate via a heuristic point-grouping stage, %after which, candidate object features are derived using a point processing network such as PointNet \cite{qi2017pointnet}, 
\cite{liu2021group} uses a grouping-free approach for detecting objects in a scene point cloud. Instead of obtaining a candidate object feature from a heuristically-grouped set of points (also called "votes"), candidate features are computed by neurally estimating the contribution of each point to the object candidate using attention mechanism. \\
%

Note that all the above works have been discussed in the context of indoor scenes, which is the focus of this report. There exist impactful works that have been developed in the context of outdoor scenes, specifically on the KITTI dataset \cite{geiger2013vision}, such as PointRCNN \cite{shi2019pointrcnn}, PointPillars \cite{lang2019pointpillars}, CenterPoint \cite{yin2021center} that operate on the 3D point cloud of the scene and are able to predict a 3D bounding box for scene objects. In theory, these architectures could very well be extended to 3D indoor scenes, but supporting experiments have not been presented.

%
\textbf{Discussion}
With an anticipated shift from feature-engineered methods \cite{song2014sliding, ren2016three, sedaghat2016orientation} to deeply learned ones \cite{song2016deep, qi2019deep, qi2020imvotenet, zhang2020h3dnet, liu2021group}, 3D object detection in indoor scenes has drawn significant research interest over the years, leading to improved performances of proposed approaches. While some of these methods employ RGB images for 2D object detection \cite{qi2020imvotenet} as an intermediate step for localizing object centroids in 3D, others do not make use of any scene image, and operate directly on the 3D scene point cloud. 

\agp{ \emph{Key factors.} As with any task in 3D, the underlying model for solving 3D object detection is governed by the choice of data representation. Assuming good quality indoor scene data at hand, extracting rich features from the 3D representation plays a critical role in the success of 3D object detection algorithms. The model should be designed to encode contextual scene information, either explicitly as done in sliding window techniques used in \cite{song2014sliding, song2016deep}, or encoding contextual relations as done in \cite{ZhangBKIX17, huang2018cooperative, FengGWZM21}, or implicitly as done in transformer-based networks. Encoding such contextual information proves useful when the input scene contains noise or occlusion and clutter. This means that the extracted features should encode spatial and semantic scene information to facilitate accurate object localization in the form of a detected 3D bounding box (location, size, and orientation). %These key aspects determine the performance of 3D object detection algorithms. This leads us to the next question: "Based on the methods discussed above, which model should I borrow/build upon?". We answer this below.\\
\newline
\emph{Which neural model to use?} Since contextual information is a strong cue in building successful 3D object detection algorithms, especially in the presence of noise and/or occlusion and clutter, the desired model should encode rich dependencies between different objects in a scene. Rings a bell? -- Transformer models. They are designed to capture long-range dependencies via the self-attention mechanism. However, they require a \emph{sequence} of inputs. For indoor scenes, this sequence can be thought of, for example, as a collection of points from a point cloud that is either representing a raw scan of an indoor scene or a processed/encoded/featurized version of the raw scan. In addition, due to their ability to capture long-range dependencies, transformers can be employed on large-scale scenes without the loss of spatial information, as opposed to when using convolutional architectures with or without specially designed modules. This is evident from \cite{liu2021group}. The downside of transformer models is that the intermediate process cannot be traced as well as in the case of CNNs (ex. being able to visualize the intermediate layers and activation maps). There is an accuracy and interpretability trade-off with transformers, but given the improved performance, they are a good starting point.\\
\newline
\emph{Good-to-have properties}} A strongly desired property in 3D deep learning is rotation equivariance. Accounting for equivariance to object rotations in 3D scenes, not at the global input level, but rather at the object level, is an interesting future direction -- attempts have been made to take into account object rotations when developing a 3D object detector \cite{ren2016three, sedaghat2016orientation}, but has not been explored by deeply learned methods. Since we are discussing about indoor scenes, object rotations are invariably around the gravity axis. 
Recently, \cite{yu2022rotationally} propose a rotationally equivariant 3D object detector, which is able to detect bounding box that are equivariant to the object pose. But even this work accounts for object rotations along the gravity axis alone. Theoretically, it may be easy to extend the framework in \cite{yu2022rotationally} to SO(3) rotations, but many fundamental issues may need to be solved in practice. Developing a 3D object detector that is equivariant to SO(3) rotations invariably begs the question:``Are there robust shape descriptors that are rotation-equivariant?".


\subsection{3D semantic scene segmentation}
\label{subsec:3d_ssg}
\input{Tables/3d_scene_seg}

%\cite{qi2017pointnet, qi2017pointnet++, dai20183dmv, thomas2019kpconv, wang2019dynamic, li2019deepgcns, zhao2021point}\\

A more in-depth understanding of indoor scenes, beyond 3D object detection, involves segmenting objects based on their semantics. An even comprehensive 3D indoor scene understanding pushes segmentation further, going into \emph{instance} segmentation (not simply semantic). 
\revision{
Indoor scenes contain a variable number of objects that occur in different positions and orientations. Moreover, some subscenes may contain identical sets of similar/identical objects, which can simply be represented by a single model. Determining the spatial extent of objects in an indoor scene (i.e., segmentation) in the presence of different categories with varying number of model instances, geometries, and rotation distributions is quite challenging. This problem also is related to object detection, since for scene segmentation, the underlying models will need to implicitly reason about objects in a scene, allowing for fine-grained localization that result in segmenting the overall object.}  

Most works in the area of 3D indoor scene understanding restrict themselves to semantic segmentation, although there are some works that tackle the instance segmentation problem. Such works primarily build on the intuitions of semantic scene segmentation networks. As such, we cover notable works that propose methods for semantic segmentation, all of which use point clouds as the choice of scene representation. Table \ref{tab:3d_scene_seg} lists notable works on 3D semantic segmentation in indoor scenes.
%
\newline
%
\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth, height = 0.6\linewidth]{Figures/scene_analysis/segmentation/3dmv.png}
    \caption{Network architecture for semantic scene segmentation, as proposed in \, cite{dai20183dmv}. It is composed of a 2D network and a 3D one. A 2D CNN extracts features from aligned images of a scene for which a geometric reconstruction is also performed from RGB-D scans. These 2D CNN features are mapped to 3D space using a differentiable back-projection layer. Features from multiple views are max-pooled on a per-voxel basis and fed into a stream of 3D convolutions, along with the reconstructed 3D geometry. Finally, both 3D streams are joined and the 3D per-voxel labels are predicted. The whole network is trained in an end-to-end fashion.}
    \label{fig:3dmv}
    \vspace{-15pt}
\end{figure}
%
\textbf{Point cloud-based techniques.}
Qi et al. \cite{qi2017pointnet} propose the very first point-cloud processing network, PointNet, that can be used for 3D semantic segmentation on shapes and scenes. It has a unified framework (supervised) for object classification and segmentation. By design, the semantic segmentation network of PointNet is an extension of the classification network which takes \emph{n} points as input, applies transformations on the input as well as intermediate feature, and then aggregates point features by max pooling; see Figure \ref{fig:point_net} for an overview. Experiments were performed on the Stanford 3D semantic parsing data which contains 3D scans of indoor environment with semantic annotations per point. During training, random crops with 4096 points coming from a room in the dataset is passed through the network which learns to assign a semantic label to each point (segmentation is essentially a classification task on each point).
During test time, all points forming a room are input to the system and semantic labels are obtained.\\

PointNet++ proposed by Qi et al. \cite{qi2017pointnet++} builds on top of PointNet to further improve semantic scene segmentation. They propose a hierarchical feature learning architecture that uses PointNet as a feature processing block. While PointNet uses a single max pooling operation to aggregate the whole point set, PointNet++ builds a hierarchical grouping of points and progressively abstracts larger and larger local regions along the hierarchy. This leads to better semantic scene segmentation. 
% \manyi{
\revision{
However, the max pooling operation used to aggregate features in local neighborhood regions often causes loss of information. PointCNN\cite{LiBSWDC18} proposed an $\chi$-conv operator to adapt the convolutional networks for point clouds. Specifically, to aggregate the local region feature of each point spanned by its K nearest neighbors, the network predicts an $\chi$-transformation matrix to weight and permute the per-point features, which is then processed using element-wise product and sum operations present in a typical convolution operation.
} 
In continuation with point convolutions, Thomas et al. \cite{thomas2019kpconv} introduce \emph{KPConv}, a convolution operation that operates on point clouds, taking radius neighborhoods as inputs and processing them with weights spatially located by a small set of kernel points. A deformable version of this convolution operator is also proposed that learns local shifts, effectively deforming the convolution kernels to make them fit the point cloud geometry. They demonstrated an improved performance on semantic segmentation which could be attributed to the flexibility offered by deformable KPConv.

Wang et al. \cite{wang2019dynamic} propose a supervised dynamic graph convolutional neural network (DGCNN) that uses PointNet as the backbone network, and demonstrate the application of their proposed method for semantic scene segmentation. The key idea is to \emph{compute} point graphs at every layer and applying \emph{edge convolutions} that are invariant to neighbor ordering. Point graphs are computed using k-nearest neighbor (based on L$_{2}$ distance) between points. The dynamic nature of graph computation at every layer of the graph convolution network enables them to capture better local and global features, leading to improved semantic scene segmentation results. Li et al. \cite{li2019deepgcns} propose a dilated version of graph convolution neural networks, which enables them to capture global features better, which is demonstrated by the results of semantic scene segmentation. 
% \manyi{

\revision{
In contrast to these sparse graphs connecting the center point and its neighbors, Zhao et al. propose PointWeb\cite{ZhaoJFJ19}, which builds dense, fully connected graphs in local regions and processes them using the Adaptive Feature Adjustment (AFA) module. This module predicts the impact of neighborhood points by adaptively aggregating contextual information on graph edges. Further, Zhou et al. \cite{ZhouFFW0L21} propose an adaptive graph convolution (AdaptConv) that generates adaptive kernels for points within a local region, rather than weighting the features based on fixed/isotropic kernels. On the other hand, Cheng et al. \cite{ChengHXY21} propose SSPC-Net, a semi-supervised method for 3D point cloud segmentation, which partitions the point clouds into super-point graphs, then dynamically propagates information from the super-point labels and uses the coupled attention mechanism to enhance the super-point features for more accurate segmentation.
}
% }
\\

%
In 3D-SIS \cite{hou20193d}, instance segmentation on 3D scans is performed by learning from both color and geometry input obtained from real RGB-D scans. Specifically, the proposed learning framework has two branches -- one that uses color images corresponding to reconstructed scan geometry, and the second one uses 3D point cloud reconstruction, either chunks of an indoor scene or a full one, from many different frames of RGB-D scan. The backbone for the first branch is a 2D CNN that extracts meaningful color features, which are brought to 3D using a differentiable back projection layer. The second branch uses a 3D CNN to obtain geometry features. Both the color and geometry features are joined in 3D. \\
%
In order to obtain object masks, they need to be localized. To this end, the work proposes a region proposal network to predict object bounding boxes. From these box predictions, class labels are predicted using a classification head, which are both used for informing instance mask predictions. Note that this is a strongly supervised approach. During inference, instances can be inferred on a full test scene in a single forward pass.

More recently, Zhao et al. \cite{zhao2021point} present a transformer-based architecture that serves as the backbone for many recognition and segmentation tasks on 3D point clouds, including semantic scene segmentation. The key insight driving this work is that the self-attention operator at the core of a transformer is essentially a set operator, and point clouds are essentially sets embedded in metric space. Much like \cite{vaswani2017attention}, their method, called Point Transformer, makes use of encoder and decoder branches which are stacked layers of what they call, a point transformer layer, which is roughly, a piece-wise summation and aggregation of outputs from two different linear layers and an MLP, all of which take points from the point cloud as input; see figure \ref{fig:point_transformer_layer} and \ref{fig:point_transformer_overall}. Although a supervised learning framework like all other works discussed till now, the gain comes from self-attention mechanism that learns the correlation between points in the input point cloud, outperforming state-of-the-art designs including graph-based models, sparse convolutional networks, and continuous convolutional networks.

\textbf{Voxel-based technqiues.}
Dai et al. \cite{dai20183dmv} propose a supervised multi-view prediction approach for semantic scene segmentation. The goal of their method is to infer semantic class labels on per-voxel level of the grid of a 3D reconstruction. To achieve this, they propose a 2D-3D neural network that leverages both RGB and geometric information obtained from 3D scans. Their method takes as input a reconstruction of an RGB-D scan along with its color images, and predicts a 3D semantic segmentation in the form of per-voxel labels; see Figure \ref{fig:3dmv} for an overview. To allow for 2D features to influence the per-voxel semantic predictions, they combine the 2D features (2D convolution on multi-view RGB images centered around a voxel location in \emph{xy} plane) with the 3D ones (3D convolutions on volumetric chunks of a scene centered around a point in the \emph{xy} plane) using a differentiable back-projection layer. This joint 2D-3D network is trained in an end-to-end fashion to predict per-voxel classes, resulting in a semantically segmented scene.
%
\newline
%
\begin{figure}[!t]
    \centering
    \includegraphics[width = 0.8\linewidth, height = 0.4\linewidth]{Figures/scene_analysis/segmentation/point_transformer_layer.png}
    \caption{\emph{Point transformer layer} from \cite{zhao2021point}. This module is essentially responsible for extracting meaningful features, which are obtained from a combination of three neural sub-modules as depicted above.}
    \label{fig:point_transformer_layer}
    \vspace{-15pt}
\end{figure}
%



\textbf{Discussion}
With the introduction of PointNet \cite{qi2017pointnet}, there has been an explosion of related works that attempt to solve standard shape+scene understanding tasks -- object classification and part/semantic scene segmentation. It is observed that architectures that are built for the task of semantic scene segmentation are all based on features meant to be used for classification purposes. In recent years, sophisticated architectures have made inroads that are based on point transformer layers \cite{zhao2021point}. All in all, backbone architectures for semantic scene segmentation seem to be pretty matured, with recent efforts being invested in engineering these networks for slightly better performance. \\% limited interest and scope for proposing new architectures.
%
\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth, height = 0.6\linewidth]{Figures/scene_analysis/segmentation/point_transformer_overall.png}
    \caption{Using the point transformer layer from \ref{fig:point_transformer_layer} as the backbone, \cite{zhao2021point} propose an architecture for point cloud processing tasks such as shape classification, part segmentation and semantic scene segmentation. }
    \label{fig:point_transformer_overall}
\end{figure}
\newline

\agp{\emph{Comparisons of Point-based and voxel-based methods.}
The discussions of related works for the task of 3D semantic scene segmentation are categorized based on the data representation (point clouds vs. voxels). This is done to focus more on the effect of data representations rather than the proposed architectures, since the discerning factors w.r.t models/architectures that apply to 3D object detection (see Section \ref{subsec:obj_det}) also apply to 3D scene segmentation. 

Point cloud-based methods that operate directly on the point coordinates do not suffer from any loss of information that occurs when with voxel-based methods that discretize the underlying data into regular grids. However, voxel-based methods capture local neighborhood geometry better than the former leading to improved segmentation accuracy. That is, compared to point cloud-based methods, they are more context-aware, owing primarily to the spatial/topology awareness of the underlying representations, but are computationally intensive compared to the former. In other words, there is an accuracy vs. efficiency trade-off, which means that the choice of a 3D scene segmentation method to build upon boils down to the complexity of the scene, and the available computational resources. In this context, it is worthwhile to investigate hybrid representations.
}
A more exciting research direction, one that is directly an extension of semantic segmentation, is \emph{instance segmentation} in 3D scenes. This area allows for fine-grained understanding of scenes since we often encounter sets of identical objects in a scene. For example, a set of chairs surrounding a dining table or a set of place settings on the table. With a wide disparity in the number of instances observed, the distribution over observed rotations, and the geometric variations among instances per model within a category, the challenges are galore. Developing advanced techniques in this direction provides a deeper insight on scene understanding tasks.% of scene segmentation.


\subsection{3D scene reconstruction}
\label{subsec:scene_recon}
\input{Tables/3d_scene_recon}
\revision{
Single-view reconstruction is a severely ill-posed problem, mainly due to the lack of sufficient priors for obtaining a faithful reconstruction. Inferring a 3D structure, either for an object or a scene, from an input image is a complex process that combines low-level image cues to learn the structural arrangement of parts/objects and the high-level semantic object/scene information. Variations in the views and shading, along with variations in textures make conventional reconstruction algorithms fail. For indoor 3D scenes, the focus is more on reconstructing object arrangements than the objects themselves. The challenge here is to reason about 3D positions from a single image, while leveraging contextual information about object arrangements reflected in the input image.
}

In general, indoor 3D scene reconstruction can be categorized into two parts: room layout reconstruction and object layout reconstruction.  Room layout reconstruction deals with recovering the spatial layout of the walls of a room, whereas object layout reconstruction involves recovering the spatial arrangement of 3D objects. We limit the scope to reconstructing object arrangements in this section (there is rich literature on reconstructing the room layouts alone). The input representations for 3D scene reconstruction tasks span the entire spectrum of visual representations, the most prominent ones being RGB (D) images and point clouds. We cover 3D object layout reconstruction works from a single RGB image \cite{izadinia2017im2cad, nie2020total3dunderstanding, zhang2021holistic, huang2018cooperative, huang2018holistic, denninger20203d}, or a set of posed RGB images \cite{murez2020atlas}, or a point cloud scan of an indoor scene \cite{song2017semantic}, as summarized below and in Table \ref{tab:3d_scene_recon}.




% \textit{Object layout reconstruction}
\textbf{Image-based techniques.}
Izadania et al. \cite{izadinia2017im2cad} propose a method for reconstructing a 3D scene of an RGB image (see Figure \ref{fig:im2cad}). They make use of a pre-trained 2D object detector (FasterRCNN \cite{ren2015faster}) to detect objects in the input RGB image, and compare the box features of these 2D  detections with that obtained from multi-view renderings of a database of CAD models (ShapeNet). This comparison enables them to retrieve an approximately aligned CAD model for a detected object in the input image. This process is done for all the object categories in consideration (eight, to be precise). 
%
In parallel, a fully convolutional network (FCN) \cite{long2015fully} is trained for room layout estimation that estimates per-pixel surface labels for ceiling, floor, and walls. The FCN network is trained on annotated scenes from the LSUN database \cite{yu2015lsun}. 


In order to find the object location and scale in the x and y directions (i.e., parallel to the ground plane) in the scene, a ray is cast from a camera center through the input image pixels corresponding to the bottom four corners of an aligned CAD model cube (note that all CAD models in ShapeNet dataset are confined within a unit cube). 
%
To compute the object scale along the z axis, they compute the ratio between the length of the four vertical edges of the projected cube and the length of those edges from the ground plane to the intersection of those lines with the horizontal vanishing line. %Note that the height of the vanishing line is equal to the camera height. 
%
After estimating the 3D room geometry and the initial placement of the objects in the scene, object placements are refined by optimizing the visual similarity of the
rendered scene with that of the input image. To this end, they solve an optimization problem where the variables are the 3D object configurations in the scene and the objective function is the minimization of the cosine distance between the convolutional features obtained from the camera view rendered scene and the input image.\\
%


\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth, height = 0.5\linewidth]{Figures/scene_analysis/recon/Im2CAD.pdf}
    \caption{\emph{IM2CAD} \cite{izadinia2017im2cad} proposes a system to reconstruct a CAD modeled scene based on a single input image. The main idea is to first render CAD models from different viewpoints and match their CNN features to that of detected objects in the input image. Once CAD models are retrieved corresponding to objects in the input image, an optimization algorithm modifies places them in a scene to reflect object arrangement in the input image. Color and lighting are injected using an additional module.}
    \label{fig:im2cad}
    \vspace{-15pt}
\end{figure}


%
Huang et al. \cite{huang2018cooperative} use a strongly supervised approach for reconstructing a 3D scene for a given RGB image, in what they call, a "cooperative" manner. Instead of developing independent modules for reconstructing parts of the scene, they propose to cooperatively estimate 3D object bounding boxes, layout bounding box and the camera pose, and project the resulting 3D layout to the image plane forcing consistency between the input image and the projected image, see Figure \ref{fig:coop_sun}. Specifically, the following three cooperative losses are used: 3D box loss (\emph{directly} optimize final estimation of the 3D boxes), 2D projection loss (maintain the \emph{consistency} between 2D image and estimated 3D boxes) and physical loss (penalize the \emph{physical} violations between 3D objects and 3D room layout). This kind of cooperation is shown to improve the estimation accuracy of 3D bounding boxes, and the physical plausibility of the overall scene. Supervisory signals are obtained from the SUNRGB-D dataset \cite{song2015sun}.

Similar to \cite{huang2018cooperative}, Nie et al. \cite{nie2020total3dunderstanding} propose a supervised method to jointly reconstruct room layout, object poses and meshes in an indoor scene from a single RGB image as the input, termed as \emph{Total3DUnderstanding} (T3DU). Their approach consists of three parts: room layout estimation (in world coordinate system), 3D object detection (in camera coordinate system), and mesh generation (in object canonical system). The output of these three modules are embedded together in the reverse order (see Figure \ref{fig:t3du}), to establish an end-to-end joint training mechanism. The 3D object detection module makes use of an attention mechanism to obtain contextual object features (called "Relational features") for a detected 2D object in the input image. The relational features are combined with the detected 2D object features (obtained using a ResNet), and the resulting features are regressed through an MLP to get 3D bounding boxes. Room layout estimation is done similarly, where the room bounding box parameters are regressed using the 3D object detector module. Finally, a mesh generation module based on AtlasNet \cite{groueix2018papier} is employed to reconstruct 3D object meshes.  

During inference, the generated meshes in the canonical system are transformed to the camera system for viewing object bounding boxes, which are in turn converted into world coordinate system for combined interpretation with the estimated room layout bounding box. This method of training in an end-to-end fashion produced improvements over \cite{huang2018cooperative} on room layout estimation and 3D object detection, and this gain can be attributed to the incorporation of relational features in 3D object detection and room layout estimation, that take scene context into account via the attention mechanism.
\\

\begin{figure*}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/scene_analysis/recon/T3DU.pdf}
    \caption{Figure illustrates the pipeline for reconstructing a 3D scene from a single image in a supervised setting. The work is called \emph{Total3DUnderstanding} \cite{nie2020total3dunderstanding}, or \emph{T3DU} in short. Relationships between detected objects in the input image are captured using attention mechanism. Both object and room layout are recovered and represented in the form of a cuboid box. Objects are reconstrcuted using a mesh generation network from \cite{groueix2018papier}.}
    \label{fig:t3du}
    \vspace{-15pt}
\end{figure*}


\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth, height = 0.5\linewidth]{Figures/scene_analysis/recon/cooperative_sun_img.PNG}
    \caption{Single-view scene reconstruction pipeline from \cite{huang2018cooperative}. The method proposes to cooperatively estimate 3D object bounding boxes, layout bounding box and the camera pose, and project the resulting 3D layout to image plane forcing consistency between the input image and the
    projected image.}
    \label{fig:coop_sun}
    \vspace{-15pt}
\end{figure}

Building on T3DU, Zhang et al. \cite{zhang2021holistic} make improvements in the quality of generated object meshes, and reduce cases of object intersections observed in T3DU. In terms of network architecture, the method is split into two stages: initial estimation stage, and a refinement stage; see Figure \ref{fig:hol_t3du}. The initial estimation stage is the same as T3DU (Figure \ref{fig:t3du}(a)), with the only difference being the employment of a network outputting a shape code based on local implicit fields \cite{genova2020local}, instead of using AtlasNet \cite{groueix2018papier} for mesh generation. In the refinement stage, the scene is modeled as a graph to capture the scene context, where the node features are concatenation of features obtained from the three modules in the initial estimation step. The node features are updated using message passing, which are later decoded into residuals to refine the initial estimation. The refined poses are then incorporated with the object shapes decoded from shape code with LDIF \cite{genova2020local} to get the final reconstruction of the whole scene. The results show an improvement over existing relevant works which can be attributed to: (a) an improved mesh generation network, (b) the incorporation of a loss term that penalizes the physical interaction of objects (in addition to other losses) and (c) modeling scenes as graphs that helps to better capture scene context and in turn, can effectively refine the initial estimates. 


Different from the aforementioned approaches, Murez et al. \cite{murez2020atlas} present \emph{Atlas}, an end-to-end 3D scene reconstruction approach from \emph{posed images}. The method takes a calibrated monocular video as input. Image features from each frame are extracted using a 2D convolutional neural network. These features are back-projected along rays into a 3D voxel volume using known camera intrinsics and extrinsics. Feature volumes are accumulated using a simple running average. After accumulation, a 3D convolutional neural network refines the features and regresses a truncated signed distance function (TSDF). The overall approach is shown in Figure \ref{fig:atlas}. Finally, a mesh is extracted from the TSDF volume using marching cubes. Additionally, semantic labels can be predicted by adding a classification head to the 3D CNN. This approach demonstrated superior quality of reconstructions on challenging long-frame temporal sequences with unobserved geometry, despite not making use of any depth information.


A more recent work called USL \cite{Gkioxari_2022_CVPR} presents an approach to scene reconstruction without any layout supervision, albeit from multi-view images of a scene during training. Their proposed system models object shapes and scene layout to roughly mimic an input image during test time. During training, given two views of a scene, one being the input to the system and the other being the target, a 3D scene is produced for the input view based on the prior work of MeshRCNN \cite{gkioxari2019mesh}. This 3D scene is now rendered from the viewpoint of the target image, and an optimization algorithm compares object masks in the two. This helps in optimizing object arrangements thereby improving the scene layout. 

\textbf{Scan-based methods.}
In SceneCAD \cite{avetisyan2020scenecad}, a solution to scene reconstruction from RGB-D scans is proposed. The problem is broken down to that of aligning CAD models to objects in RGB-D scans. The prelude to SceneCAD is a prior work called Scan2CAD \cite{avetisyan2019scan2cad} that aims at estimating object arrangements from 3D scans by learning to align CAD models to RGB-D scans. The emphasis here is on the type of input -- RGB-D scans, which tend to be very noisy and incomplete, with no semantic information. SceneCAD solves a joint problem of estimating both object and room layout information, by capturing relationships among objects and between objects and room elements, such as walls. The end result is a lightweight digitized representation for the input RGB-D scan. Note that this is also a supervised learning approach, with supervision on class labels during object mask predictions and edge labels between graph nodes. 
Many recent approaches to single-view scene reconstruction \cite{kuo2020mask2cad, kuo2021patch2cad, gumeli2022roca} propose similar proxy solutions based on shape recovery of detected 2D objects in the input image via CAD model alignment.

%
\begin{figure*}[!t]
    \centering
    \includegraphics[width = 0.8\linewidth, height = 0.25\linewidth]{Figures/scene_analysis/recon/holistic_t3du.pdf}
    \caption{Figure illustrates various modules present in reconstructing a 3D scene from a single image as proposed in \cite{zhang2021holistic}. It is a supervised learning framework. The work mainly builds on Total3DU \cite{nie2020total3dunderstanding}, with the major difference being the use of implicit representations for objects in a scene. In addition, a graph neural network is employed on the scene objects, allowing to capture better contextual information. Room and object layout are represented using box cuboids, and objects are reconstructed using LDIF \cite{genova2020local}.}
    \label{fig:hol_t3du}
    \vspace{-15pt}
\end{figure*}


\textbf{Discussion}
3D supervision is hard to obtain, which necessitates the exploration of challenging tasks to scene reconstruction from one or more images. In order to truly reconstruct an indoor 3D scene, both room layout (walls and their arrangement), and object layout (spatial placements of objects in a room) should be recovered, which are non-trivial to solve. In 3D vision, a lot of effort has been put in recovering room layouts from a single image, starting from \cite{hedau2009recovering} to more recent works like \cite{dasgupta2016delay, lee2017roomnet, zou2018layoutnet, huang2018holistic, yang2019dula}. Model-based room layout reconstruction algorithms such as the ones proposed by \cite{hedau2009recovering, mallya2015learning} are limited by hand-crafted features based on one/few properties of physical existence. Learning from data, however, can uncover the full potential of realizable results, allowing to explore further in that direction.

For object layout reconstruction from single/multiple images or 3D scans, two major approaches exist -- (1) learning contextual placements of objects, or (2) aligning CAD models to the input. The first approach is mainly a supervised setting, based on attention mechanism \cite{nie2020total3dunderstanding} or message passing \cite{zhang2021holistic} since they need a notion of what plausible placements look like. In addition to recovering object layouts, these works also perform reconstruction at the object level, which may not be ideal for visualizing results since single-view reconstruction for objects is a research area in itself. A more recent work \cite{Gkioxari_2022_CVPR} does not make use of layout supervision, but gains additional training information by making use of \emph{multi-view} images of the same scene, which compensates for the lack of layout-level supervision. 

The second approach is an ad-hoc setting, moving towards unsupervision at the layout level, where the goal is to simply align CAD models from a database to detected objects in the input image \cite{izadinia2017im2cad} or input 3D scans \cite{avetisyan2020scenecad, avetisyan2019end, avetisyan2019scan2cad, kuo2020mask2cad, kuo2021patch2cad, gumeli2022roca, maninis2022vid2cad}. These approaches are more closer to works that estimate object poses from a single input image, with an added component of optimizing for object placements that reflect the input image/scan. Overall, an unsupervised learning framework that could be trained from a single input image is missing.

%There are some ad-hoc CAD-scene object alignmnet works, such as Mask2CAD, Patch2CAD, ROCA. Also, discuss about the proximity of this to pose estimation, which is pretty wide in scope.

%Online scene reconstruction -- Mask2CAD, Patch2CAD


\subsection{3D scene similarity}
\label{subsec:scene_sim}
%\input{Tables/3d_scene_sim}

In visual computing, a metric is used to compare different data representations such as two images, meshes, voxels etc., and provide a measure of closeness or similarity between samples in consideration. As a result, they find applications in database retrieval, data clustering, and evaluating the diversity of generative models. 


Similarity metrics for 3D shapes (Chamfer Distance, IoU, Light Field Distance etc.) and 2D images (L2 distance, PSNR) make an underlying assumption that the data being compared can be globally aligned.
%
However, the concept of global alignment between two 3D scenes, even if they are of the same type, is rather weak since there is no "correct" sequence of populating 3D objects in a space to compose a plausible scene, where same objects can be placed quite differently in two scenes. In addition, scene comparison is complicated when the two scenes (of the same type) have different 3D objects, both semantically and geometrically. As such, developing a metric for comparing 3D scenes is quite challenging, but interesting at the same time due to many degrees of design freedom. %We summarize notable such works below and provide a comprehensive overview in Table \ref{tab:3d_scene_sim}.\\
%
\newline
%
 \begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/scene_analysis/recon/atlas.pdf}
    \caption{End-to-end training pipeline for 3D scene reconstruction from posed images \cite{murez2020atlas}. The method takes a monocular video as input and extracts 2D CNN features from each frame, which are back-projected to 3D voxel grids using known camera information. A 3D CNN refines the features and regresses a TSDF function, from which a scene mesh is extracted using the marching cubes algorithm.}
    \label{fig:atlas}
    \vspace{-15pt}
\end{figure}

%
\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/scene_analysis/similarity/graph_kernel.png}
    \caption{\emph{Graph Kernels} in \cite{fisher2011characterizing} is a method for characterizing the structural relationships between two subscenes. In the figure above, a scene is represented as a relational graph shown on the left. Two types of relationships are considered, as indicated by the arrows. The figure on the right shows an example of the process involved in finding similarity between two subscenes using graph walks. Both walks in each scene are rooted at the lamp
    node. The two walks are compared by taking the product of kernel evaluations for their constituent nodes and edges.}
    \label{fig:GK}
    \vspace{-15pt}
\end{figure}
\textbf{Graph Kernels.}
Fisher et al. \cite{fisher2011characterizing} was the first work to develop a method to measure 3D scene similarity, called \emph{Graph Kernels}. Specifically, they characterize 3D scenes using graphs (see Figure \ref{fig:GK} left), where the edges of a graph encode physical proximity relationships (such as support, contact, enclosure) between objects (nodes) in a scene and the nodes correspond to objects in the scene, which encode the geometric information of the objects. With such graph-based representation of scenes, a kernel is defined for comparison of two relationship graphs in a way that similarities between the graph nodes and edges are computed and accumulated to produce an overall similarity of two graphs (see Figure \ref{fig:GK} right). \\
%
\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/scene_analysis/similarity/ibs_a.png}
    \caption{\emph{Interaction Bisector Surface (IBS)} \cite{zhao2014indexing} is a rich representation between objects in a scene that describes topological and geometric relationships between objects in a scene. IBS is the set of points equidistant from two sets of points sampled on different objects, shown as the blue-colored surface above.}%  It is an approximation of the Voronoi diagram for objects in a scene.}
    \label{fig:IBS-a}
    \vspace{-15pt}
\end{figure}
%

\textbf{Interaction descriptors.}
Zhao et al. \cite{zhao2014indexing} propose a scene relationship descriptor, called Interaction Bisector Surface (IBS), to characterize complex relationships in a scene, or rather, a sub-scene. IBS describes topological (wrapped in, linked to or tangled with) as well as spatially proximal relationships between objects (see Figure \ref{fig:IBS-a}). IBS is defined as the set of points that are equidistant from two objects, which form an approximation of the Voronoi diagram for objects in the scene.  IBS is used to define a similarity metric between objects, which is then used to group similar objects in a bottom-up manner to automatically construct hierarchies. Unlike \cite{fisher2011characterizing}, IBS does not make use of object labels, and instead, focuses on modeling interaction between objects where spatial relationships between objects are characterized by topological and geometric features. Thus, IBS enables content-based relationship retrieval based on interaction similarity. Figure \ref{fig:ibs retrievals} provides an example of content-based relationship retrieval based on IBS. \\

\textbf{Object-centric descriptor.}
Xu et al. \cite{xu2014organizing} present a method to organize a heterogeneous collection of scenes by what they call \emph{focal points}. The key insight in this work is that analyzing complex and heterogeneous scenes in a collection is difficult without references to certain points of attention or focus. \emph{Focal points} provide such points of attention against which two or more complex scenes could be compared. 
Specifically, \emph{focal points} are defined as representative substructures in a scene collection, using which similarity distances between scenes could be computed, see Figure \ref{fig:focal points a} for an illustration. Identifying focal points from a collection of scenes is a problem that is coupled with clustering scenes based on a common point of reference. To solve the coupled problems of focal
point extraction and scene clustering, a co-analysis algorithm that interleaves frequent pattern mining and subspace clustering is presented to extract a set of contextual focal points that guide scene clustering from within the collection. This is shown in Figure  \ref{fig:focal points b}. This co-analysis-based method of focal point extraction extends itself towards scene comparison (retrieval), and exploration of a heterogeneous collection of scenes. 
%

\textbf{Learning on scene graphs.}
Recently, \cite{wald2020learning} propose a neural network that infers a semantic scene graph from an instance-segmentation of a 3D scene, represented as a point cloud. Leveraging these \emph{learned} semantic scene graphs, a 3D scene retrieval is performed where the objects in the scene represent the nodes in the learned graph, and edges represent generic connection as well as semantic relations (such as: next to, lying on, close by) between scene objects. This is achieved by graph matching, not using any neural network, but using a deterministic similarity function based on two types of metric -- Jaccard coefficent and Szymkiewicz-Simpson (SS) coefficient. When matching two graphs G and G$^'$, they combine the similarity metric of the object semantics, generic
node edges E as well as semantic relationships R. 

Since the semantic graphs are rich with relational semantics between objects, and the similarity function based on either the Jaccard coefficient or the Szymkiewicz-Simpson coefficient can provide meaningful similarity scores, especially SS coefficient when the two scenes A and B have very different sizes, one can use this retrieval method to find rooms that fulfill certain requirements such as the availability of objects e.g. meeting room with a TV, whiteboard.


\textbf{Discussion}
Efficient retrieval of 3D scenes is helpful in visualizing interior design possibilities. The query to such systems can be in different forms -- 2D image, text input, a sketch, a scene graph, a sequence of attributes, etc., each of which poses unique challenges. The central goal to this problem is to define a similarity function that captures the space of scenes based on either pre-defined properties (such as focal-centric themes) or incorporates as many attributes of a scene as possible directly from the data. 

\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/scene_analysis/similarity/ibs_retrieval.png}
    \caption{Retrievals results using IBS features \cite{zhao2014indexing} -- In the query scene on the left, a desk, overlayed using its bounding box, is the query object for IBS algorithm. On the right are the scenes ordered based on their similarity, where the red object is the retrieved object with a similar context to the query desk.}
    \label{fig:ibs retrievals}
    \vspace{-15pt}
\end{figure}

As discussed above, graph neural networks (GNN) appear to sit comfortably in becoming the preferred tool to tackle 3D scene retrieval problems. In recent years, \emph{neural} graph matching networks \cite{patil2021layoutgmn} have been shown to effectively capture similarity on 2D layouts, albeit with inherent sluggishness due to dependent graph embeddings (embedding of one graph is equally governed by the other graph in a pair). This could be extended to 3D scenes, where the focus should be on efficiently matching scene graphs in a large database, using hashing techniques. 


==> 6-new_trends_in_scene_synthesis.tex <==
\agp{
\section{New Trends in 3D Indoor Scene Synthesis}
\label{sec:new_trends}
\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/scene_synthesis/neural_synthesis/scene_former.png}
    \caption{\emph{SceneFormer} \cite{wang2020sceneformer} uses a transformer to generate new scenes in an autoregressive manner, where a scene is represented by an ordered set of objects. In addition, it consumes a floor image, both during train and test time.}
    \label{fig:scene former}
    \vspace{-15pt}
\end{figure}

In recent years, neural scene rendering \cite{mildenhall2021nerf}, diffusion models \cite{sohl2015deep, ho2020denoising}  and CLIP-based models \cite{radford2021learning} have gained a lot of traction for generating novel data samples. They have been predominantly employed in the 2D domain, with only recent exploration for 2D-to-3D generation \cite{gao2022get3d, poole2022dreamfusion} on single-object images. Leveraging these models for 3D indoor scenes is an under-explored direction mainly due to the complexity of the scene structures. Below, we present relevant recent works that use these newer techniques for synthesizing indoor scenes. %We only provide these as pointers

\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/scene_synthesis/neural_synthesis/ATISS.png}
    \caption{\emph{ATISS} \cite{paschalidou2021atiss} poses the scene synthesis task as one of unordered set generation. Given a room type and its shape (in the form of a top-down floor image), it generates plausible furniture arrangements in an autoregressive, permutation-invariant fashion using a transformer.}
    \label{fig:ATISS}
    \vspace{-15pt}
\end{figure}

%Indoor scene synthesis, on the other hand, is not merely about generating novel views of a scene. Rather, it has to do with how objects are arranged in a given space and if their arrangement can be manipulated, even if it is limited to a few objects in the scene. Recent advancements in generative modeling has led to the emergence of modern tools, such as Diffusion models \cite{sohl2015deep, ho2020denoising} and CLIP \cite{radford2021learning}, that are capable of generating high-quality data samples, mainly in the 2D domain \cite{saharia2022photorealistic, ho2022video}. This direction of research has seen an explosion of works in the 2D domain, but not so much in 3D, let alone on 3D indoor scenes.

%To this end, we survey recent works using NeRF \cite{mildenhall2021nerf}, Diffusion \cite{sohl2015deep, ho2020denoising}  and CLIP-based models \cite{radford2021learning} that modulate object arrangements or hallucinate/fill/extrapolate views in indoor scenes to generate novel such samples.

\textbf{Using Radiance Fields}
The basic idea in neural rendering is to first sample spatio-temporal coordinates with respect to a given 3D scene, feed it through a neural network to recover radiance/signed-distance fields and employ a differentiable forward map (such as sphere tracing or volume rendering) that outputs a novel view RGB image (see \cite{xie2022neural} for a detailed report).
Using these radiance fields to hallucinate scene geometry or to manipulate object arrangements allows their employability for indoor scene modeling applications. 

%Indoor scene synthesis, on the other hand, is not merely about generating novel views of a scene. Rather, it has to do with how objects are arranged in a given space and if their arrangement can be manipulated, even if it is limited to a few objects in the scene

%For a realistic experience in AR/VR applications, it is desired that users be assisted with necessary technology to manipulate partial/entire scenes, while maintaining the overall appearance. Neural rendering techniques provide a promising solution, although they are mainly designed for novel-view synthesis. 
To this end, \cite{devries2021unconstrained, yang2021learning} present some of the early works on using radiance fields for scene hallucination/completion and scene editing, respectively. Yang et al. \cite{yang2021learning} develop a neural rendering system that enables editing on real-world scenes by learning an object-compositional neural radiance field. The main idea is to use two separate branches to encode the scene, one to process the scene background and the other to process the constituent objects, both undergoing a neural rendering pipeline of their own. In doing so, the system runs a neural radiance field pipeline on the object branch that takes as inputs object voxel features and an object activation code, allowing scene edits at the object level based on the object activation code.

DeVries et al. \cite{devries2021unconstrained} make use of the radiance fields to learn scene priors from which novel scenes can be sampled. Specifically, they train a GAN in which the generator learns to decompose scenes into a collection of many \emph{local} radiance fields that can be rendered from a freely moving camera. The generator of this proposed GAN tries to learn a distribution of novel view images (using a NeRF model) that is similar to the prior distribution. The discriminator is tasked to classify the images at the output of the generator to be fake. Once trained on many diverse scenes and viewpoints, a novel scene sample can be generated using a random vector that can hallucinate parts of a scene captured in the training images.

\cite{wang2022neuralroom} propose NeuralRooms to reconstruct indoor scenes (represented by meshes) from unposed multi-view 2D images based on neural radiance fields. The main motivation of this work is that shape-radiance ambiguity and the presence of texture-less regions in indoor scenes make it difficult to faithfully reconstruct them using multi-view stereo (MVS) algorithms or using NeRF models. To address this issue, they propose a two-part learning framework wherein the first part makes use of a MVS algorithm \cite{schonberger2016structure} (ensuring the accuracy of texture-rich and edge areas) and a normal estimation network \cite{bae2021estimating} (ensuring completeness of texture-less regions) to acquire geometry prior. The input RGB images and the geometry prior are used in a neural rendering-based surface reconstruction pipeline. Finally, ray-tracing on the reconstructed scene is done with TSDF fusion to obtain a 3D mesh for the reconstructed indoor scene.

\begin{figure*}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/new_trends/diffusion_model/lego_net.png}
    \caption{Denoising process of LEGO-Net \cite{wei2023lego}(left) and the backbone transformer (right) performing the denoising process. LEGO-Net takes the current scene state and iteratively modifies the scene state by computing denoising gradient towards the clean manifold. The transformer on the right transformer takes the scene attributes of the current state and outputs 2D transformations of each object.}
    \label{fig:lego-net}
    \vspace{-15pt}
\end{figure*}

\textbf{Using Diffusion and CLIP-based models}
Unlike in the 2D domain, the deployment of diffusion models for modeling 3D indoor scenes has not seen much activity. To the best of our knowledge, the recent works of Lego-Net \cite{wei2023lego} and \cite{lei2022generative} are the only work devoted to this task. 

Lego-Net \cite{wei2023lego} develops a denoising diffusion model to learn the rearrangement of objects in a messy indoor scene, where, similar to ATISS, a scene is represented by an unordered set of objects and their transformations. The underlying model that is used is a transformer. Given an input messy scene, the transformer iteratively computes the denoising gradient towards the clean manifold, until a so-called regular state is reached; see Figure \ref{fig:lego-net}. Note that the denoising process is not driven by any end goal state, and the concept of an end goal state is not made use of in this work. At each step of the denoising process, the transformer takes scene attributes of the current state and outputs 2D transformations of each object that would make the scene ``cleaner". Training this model takes place in a reverse fashion where clean scenes are perturbed to make them messy. 

Lei et al. \cite{lei2022generative}, on the other hand, propose to synthesize an indoor scene via incremental inpainting. They represent indoor scenes as RGBD images. Given a sparse set of multi-view RGBD images, the goal is to generate a coherent 3D scene mesh by predicting RGBD frames along a \emph{novel} camera trajectory. To this end, they first fuse the input view images into an initial mesh, which is then rendered to get an incomplete, hole-present image of the scene. This incomplete scene is then inpainted using a RGBD diffusion model which is back-projected to the 3D domain to get a 3D mesh. This mesh is integrated with the very initial mesh to get a new mesh. This process takes place in an iterative fashion, eventually generating a novel indoor scene.

CLIP \cite{radford2021learning} is a popular text-to-image generative model capable of producing novel 2D images from text prompts. In the 3D domain, CLIP has been used to generate 3D shapes as shown in \cite{sanghi2022clip, sanghi2022textcraft}. Its extension to generating 3D indoor scenes is not straightforward owing to the presence of multiple objects. CLIP-Layout \cite{liu2023clip} presents the first work that leverages a CLIP model to synthesize 3D indoor scenes. 

Similar to ATISS \cite{paschalidou2021atiss}, CLIP-Layout \cite{liu2023clip} adopts an auto-regressive approach for indoor 3D scene synthesis, but the synthesis is now additionally constrained on a text input that acts as a style description prompt. This work also encodes a 3D scene as an unordered set of objects and their transformations, and the underlying machinery is based on a transformer model. The text prompt is encoded using a CLIP encoder \cite{radford2021learning}, which takes eight view-renderings of a 3D scene as input and outputs a 512-dimensional vector, which is then concatenated with all other object-plus-floor features extracted using the transformer as done in ATISS. Note that a pre-trained text-to-image CLIP encoder is used during the training phase. This allows the representation of fine visual details of each furniture instance while remaining agnostic to object encoding format. Sample results are shown in Figure \ref{fig:clip_layout}.

\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{Figures/new_trends/clip_models/CLIP_layout.png}
    \caption{CLIP-Layout \cite{liu2023clip} takes a floorplan and a text prompt as conditions for style descriptions, and generates plausible, diverse 3D indoor scenes that are stylistically consistent, adhering to the input text prompt.}
    \label{fig:clip_layout}
\end{figure}
}

==> Tables/3d_scene_sim.tex <==
%\begin{figure*}[h]
\begin{table*}[!t]
\centering
\begin{tabular}{|p {1  cm}|p {1.5  cm}|p {1.4  cm}|p {1.5  cm}|p {1.75  cm}|p {2  cm}|p {2.3  cm}|p {2.5  cm}|}
\hline
\textbf{Related Work} & \textbf{Learning Framework} & \textbf{Scene rep} & \textbf{Backbone} & \textbf{Input} & \textbf{Output} & \textbf{Dataset} & \textbf{Evaluation Metric(s)}\\[0.5 ex]
%
\hline
\cite{fisher2011characterizing} & - & - & - & - & - & - & - \\
%
\hline
\cite{zhao2014indexing} & - & - & - & - & - & - & - \\
%
\hline
\cite{xu2014organizing} & - & - & - & - & - & - & - \\

%
\hline
%
\end{tabular}
%\vspace{-0.25 em}
\caption{Notable works on \textbf{3D indoor scene similarity} -- \emph{Input} and \emph{Output} refer to the input consumed by the \emph{Backbone} and its output, respectively.}
\label{tab:3d_scene_sim}
\vspace{-15pt}
\end{table*}
%\vspace{-2 em}
%\end{figure*}


==> Tables/datasets.tex <==
%\begin{figure*}[h]
\begin{table*}[!t]
\centering
\begin{tabular}{p {1.6  cm}|p {1.4  cm}|p {1.4  cm}|p {1.5  cm}|p {1.5  cm}|p {1.  cm}|p {1.2  cm}|p {1.5  cm}|p {1.5 cm}}
% \hline
\toprule
\textbf{Name} & \textbf{Data} & \textbf{Source} & \textbf{Coverage} & \textbf{Capture} & \textbf{\#scenes} & \textbf{\#CAD models} & \textbf{Model Textures} & \textbf{3D Annotation}\\[0.5 ex]
% % SUN 360 dataset website not available, hence not included
    % \hline
    \midrule
    SUN 3D \cite{xiao2013sun3d}  & Registered RGB-D & Real scans & Perspective & Hand-held video & $254$ & - & No texture & Raw PCD \\
    % \hline
    SUN RGB-D \cite{song2014sliding}  & Registered RGB-D & Real scans & Perspective & Hand-held video & $10779$ & - & No texture & Raw PCD \\
    % \hline
    UZH 3D dataset \cite{UZHdataset} & Registered PCD & Real/Synth & Scan & Tripod & 53 & - & No texture & PCD\\
    %
    % \hline
    % bundle fusion dataset link not available, hence not included here
    ETH 3D dataset \cite{ETH3D} & Registered RGB & Real scene images & Perspective & Tripod & 898 & - & No Texture & PCD\\
    %
    % \hline
    Matterport3D \cite{chang2017matterport3d} & Registered RGB-D & Real scans & Panoramic & Tripod & $2,056$ & - & Rec. from scans & Raw Mesh\\
    %
    % \hline
    ScanNet \cite{dai2017scannet} & Registered RGB-D & Real scans & Perspective & Hand-held video & $1,506$ & $296$ & Rec. from scans & Raw Mesh \\
    %
    % \hline
    CRS4/ViC dataset \cite{CRS4} & Registered RGB & Real scene images & Panoromic & Tripod & 191 & - & No texture & - \\
    %
    % \hline
    Replica dataset \cite{replica19arxiv} & CAD model & Synth & All & Manual modeling & 18 & - & RGB texture camera & Mesh\\
    %
    % \hline
    Structured3D dataset \cite{zheng2020structured3d} & CAD model & Synth & All & Manual modeling & 3500 & - & No texture & 3D structure\\
    % \hline
    NYU Depth v2 \cite{silberman2012indoor} & Registered RGB-D & Real scene images & Perspective & Hand-held video & 1449 & - & No texture & RGB-D \\
    %
    % \hline
    TUM \cite{sturm2012benchmark} & Registered RGB-D & Real scene images & Perspective & Hand held video & 39 & - & No texture & RGB-D \\
    %
    % \hline
    %S3DIS \cite{armeni20163d} &
    3DSSG \cite{wald2020learning} & PCD & Real scenes & All & Hand-held device & 1482 & - & Rec from scans & Mesh + scene graph\\
    %
    % \hline
    SceneNN \cite{hua2016scenenn} & RGB-D & Real scenes & Perspective & Hand-held device & 100 & - & Rec. from scans & Mesh\\
    %
    % \hline
    Scan2CAD \cite{avetisyan2019scan2cad} & Mesh & Real scans & All & Manual modeling & 1506 & 3049 & No texture & Mesh \\
    %
    % \hline
    OpenRoom \cite{li2021openrooms} & RGB-D & Real scans & Perspective & Hand-held decide & 1287 & 44 & UV mapping & Mesh \\
    %
    % \hline
    SceneNet \cite{handa2016understanding} & Mesh & Synth & All & Manual modeling & 57 & 3699 & No texture & Mesh \\
    %
    % \hline
    InteriorNet \cite{li2018interiornet} & RGB & Synth & Perspective & Manual modeling & - & - & No texture & N/A \\
    %
    % \hline
    Hypersim \cite{roberts2021hypersim} & RGB & Synth & Perspective & Manual modeling & 461 & - & Per pixel color & RGB-D \\
    %
    % \hline
    3D-FRONT \cite{fu20213d} & Mesh & Synth & All & Manual modeling & 18968 & 13151 & Professional & Mesh\\
    \bottomrule
\end{tabular}
%\vspace{-0.25 em}
\caption{A summary of publicly available 3D indoor scenes datasets along different axes that include high-level details such as the physical mode of capture to low-level ones such as the kinds of annotations on the scene and the number of CAD models/ scenes. \textit{\#scenes} indicates number of rooms/scenes populated with 3D furniture objects, \textit{N/A}=``Not Applicable", \textit{PCD}=``Point cloud".}
\label{tab:dataset_list}
%\vspace{-15pt}
\end{table*}
%\vspace{-2 em}
%\end{figure*}


==> Tables/datasets_v3.tex <==
%\begin{figure*}[h]
\begin{table*}[!t]
\centering
\begin{tabular}{p {3.2  cm}|p {1.4  cm}|p {1.5  cm}|p {1.5  cm}|p {1.  cm}|p {1.2  cm}|p {1.8 cm}|p {1.5 cm}}
% \hline
\toprule
\textbf{Name} & \textbf{Data} &  \textbf{Coverage} & \textbf{Capture} & \textbf{\#scenes} & \textbf{\#CAD models} & \textbf{Model Textures} & \textbf{3D Annotation}\\[0.5 ex]
    % \hline
    \midrule
    \multicolumn{8}{l}{\textbf{Real scans}}\\
    \midrule
    %
    SUN 3D \cite{xiao2013sun3d}  & Registered RGB-D &  Perspective & Hand-held video & $254$ & - & No texture & Raw PCD \\
    %
    SUN RGB-D \cite{song2014sliding}  & Registered RGB-D &  Perspective & Hand-held video & $10779$ & - & No texture & Raw PCD \\
    %
    Matterport3D \cite{chang2017matterport3d} & Registered RGB-D &  Panoramic & Tripod & $2,056$ & - & Rec. from scans & Raw Mesh\\
    %
    ScanNet \cite{dai2017scannet} & Registered RGB-D &  Perspective & Hand-held video & $1,506$ & $296$ & Rec. from scans & Raw Mesh \\
    %
    Scan2CAD \cite{avetisyan2019scan2cad} & Mesh &  All & Manual modeling & 1506 & 3049 & No texture & Mesh \\
    %
    OpenRoom \cite{li2021openrooms} & RGB-D &  Perspective & Hand-held decide & 1287 & 44 & UV mapping & Mesh \\
    %
    UZH 3D \cite{UZHdataset} & Registered PCD & Scan & Tripod & 53 & - & No texture & PCD\\
    %
    3DSSG \cite{wald2020learning} & PCD & All & Hand-held device & 1482 & - & Rec from scans & Mesh + scene graph\\
    %
    SceneNN \cite{hua2016scenenn} & RGB-D & Perspective & Hand-held device & 100 & - & Rec. from scans & Mesh\\
    %
    \midrule
    \multicolumn{8}{l}{\textbf{Synthetic}}\\
    \midrule
    %
    Replica \cite{replica19arxiv} & CAD model &  All & Manual modeling & 18 & - & RGB texture camera & Mesh\\
    %
    Structured3D \cite{zheng2020structured3d} & CAD model &  All & Manual modeling & 3500 & - & No texture & 3D structure\\
    %
    SceneNet \cite{handa2016understanding} & Mesh &  All & Manual modeling & 57 & 3699 & No texture & Mesh \\
    %
    InteriorNet \cite{li2018interiornet} & RGB &  Perspective & Manual modeling & - & - & No texture & - \\
    %
    Hypersim \cite{roberts2021hypersim} & RGB &  Perspective & Manual modeling & 461 & - & Per pixel color & RGB-D \\
    %
    3D-FRONT \cite{fu20213d} & Mesh &  All & Manual modeling & 18968 & 13151 & Professional & Mesh\\
    %
    \midrule
    \multicolumn{8}{l}{\textbf{Real scene images}}\\
    \midrule
    ETH 3D \cite{ETH3D} & Registered RGB &  Perspective & Tripod & 898 & - & No Texture & PCD\\
    %
    CRS4/ViC \cite{CRS4} & Registered RGB &  Panoromic & Tripod & 191 & - & No texture & - \\
    %
    NYU Depth v2 \cite{silberman2012indoor} & Registered RGB-D &  Perspective & Hand-held video & 1449 & - & No texture & RGB-D \\
    %
    TUM \cite{sturm2012benchmark} & Registered RGB-D &  Perspective & Hand held video & 39 & - & No texture & RGB-D \\
    \bottomrule
\end{tabular}
%\vspace{-0.25 em}
\caption{A summary of publicly available 3D indoor scenes datasets along different axes that include high-level details such as the physical mode of capture to low-level ones such as the kinds of annotations on the scene and the number of CAD models/ scenes. \textit{\#scenes} indicates number of rooms/scenes populated with 3D furniture objects, \textit{N/A}=``Not Applicable", \textit{PCD}=``Point cloud".}
\label{tab:dataset_list}
%\vspace{-15pt}
\end{table*}
%\vspace{-2 em}
%\end{figure*}


==> Tables/scope_outlined.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{p {1.6  cm}|p {1.4  cm}|p {1.4  cm}|p {1.5  cm}|p {1.5  cm}|p {1.  cm}|p {1.2  cm}|p {1.5  cm}|p {1.5 cm}}
% \hline
\toprule
\textbf{Section} & \textbf{Problem Addressed} \\[0.5 ex]
% % SUN 360 dataset website not available, hence not included
    % \hline
    \midrule
    \ref{sec:layout_reps} & Scene representation \\
\end{tabular}
%\vspace{-0.25 em}
\caption{\agp{AGP to complete}}
\label{tab:scope_outlined}
%\vspace{-15pt}
\end{table}
